Improving ChatGPT Prompt for Code Generation

Automated code generation can be a powerful technique for software development, significantly reducing developers' efforts and time required to create new code by generating it automatically based on requirements. Recently, OpenAI's language model ChatGPT has emerged as a powerful tool for generating human-like responses to a wide range of textual inputs (i.e., prompts), including those related to code generation. However, the effectiveness of ChatGPT for code generation is not well understood, and the generation performance could be heavily influenced by the choice of prompt. To answer these questions, we conducted experiments using the CodeXGlue dataset to evaluate ChatGPT's capabilities for two code generation tasks, including text-to-code and code-to-code generation. We designed prompts by leveraging the chain-of-thought strategy with multi-step optimizations. Our results showed that by carefully designing prompts to guide ChatGPT, the generation performance can be improved substantially. We also analyzed the factors that influenced the prompt design and provided insights that could guide future research.

==> code/binary.tex <==
test eax, eaxjz
jz short 424BED
jmp 424D75
mov [ebp+var_1110], 1
jmp short 424C08

pop edi
mov esp,ebp
pop ebp
retn

==> code/code_annotation.tex <==
-@Service
+@Repository
public class PriceComponentRepositoryImpl implements PriceComponentRepository {
    private final PriceComponentDao priceComponentDao;
    private final PriceComponentMapper priceComponentMapper;

    @Override
    public void createPriceComponent(PriceComponent priceComponentToCreate) throws PriceComponentAlreadyExistsException {
        ...
    }
}

==> code/code_api_usage.tex <==
// target code
public long getEdgeIdByNodes(long id1, long id2){
    Node n1 = graphDb.getNodeById(id1);
    Iterator<Relationship> iter = n1.getRelationships().itertor();
    while (iter.hasNext()){
        ...
    }
}

// API usage recommendation by ChatGPT
// The provided code example is using the Neo4j Java API to retrieve an edge ID that connects two nodes with the given IDs. Here are some code examples: ...

// graphDb.getNodeById(id1): This method ... Here's an example: ...



==> code/code_completion.tex <==
// incomplete code
class MyClass:
    def __init__(self, __name, __pay):
        self.name = __name
        self.pay = __pay

    def lastName(self):

// code completion by ChatGPT
class MyClass:
    def __init__(self, name, pay):
        self.name = name
        self.pay = pay

    def lastName(self):
        return self.name.split()[-1]

==> code/code_generation.tex <==
// ground-truth for description "binds a hiberate session to the current thread"
private void bindSession(){
    SessionFactory sessionFactory=(SessionFactory)getBean("sessionFactory");
    Session session=sessionFactory.openSession();
    TransactionSynchronizationManager.bindResource(sessionFactory, new SessionHolder(session));
}

// code generation by ChatGPT
Configuration configuration = new Configuration();
built-in connection pooling
configuration.setProperty("hibernate.connection.driver_class", "com.mysql.jdbc.Driver");
...
configuration.addAnnotatedClass(MyEntity.class);
SessionFactory sessionFactory = configuration.buildSessionFactory();
Session session = sessionFactory.getCurrentSession();
session.beginTransaction();
try {
    MyEntity entity = new MyEntity();
    entity.setName("John Doe");
    session.save(entity);
    session.getTransaction().commit();
} catch (Exception e) {
    session.getTransaction().rollback();
    throw e;
} finally {
    session.close();
}

==> code/codebase_search.tex <==
// query: calculate checksum of checkpoint

// the top-1 searched code
checksum(unsigned short *buffer, int size){
    unsigned long cksum=0;
    while (size>1){
        cksum += *buffer++;
        size -= sizeof(unsigned short); 
    }
    if (size){
        chksum += *(unsigned char *)buffer;
    }
    cksum = (cksum >> 16) + (cksum & 0xffff);
    cksum += (cksum >> 16);
    return (unsigned short)(~cksum);
}

// the top-2 search code
uint16_t cksum(char *b, int len){
    uint16_t sum = 0;
    uint16_t t;
    char *e = b + len;
    b[len] = 0;
    while (b<e){
        t = (b[0]<<8)+b[1];
        sum+=t;
        if(sum<t)
            sum++;
        b+=2;
    }
    return ~sum
} 

==> code/comment_debt.tex <==
// target technical debt
// 1. do we need to update the crosshair values?
// 2. defer argument checking...
// 3. do we need to update the crosshair values?

==> code/comment_position.tex <==
protected void checkOptions() throws BuildException{
    //set the destination directory relative from the project if needed
    if (toDir == null){
        toDir = task.getProject().resolveFile(".");
    }else if (!toDir.IsAbsolute()){
        toDir = task.getProject().resolveFile(toDir.getPath()); //get path
    }
}

==> code/comment_summarization.tex <==
// target code with ground-truth "create an IIS application"
def create_app(name, site, sourcepath, apppool=None):
    pscmd = list()
    pscmd.append("New-WebApplication -Name '{0}' -
    Site'{1}'".format(name,site))
    pscmd.append(" -PhysicalPath '{0}'".format(sourcepath))
    if apppool:
        pscmd.append(" -applicationPool '{0}'".format(apppool))
    cmd_ret = _srvmgr(str().join(pscmd))
    if cmd_ret['retcode'] == 0:
        if name in list_apps(site): return True
    return False

// comment summarization by ChatGPT
// The provided code defines a Python function create_app that creates a new web application in IIS ...

==> code/comment_update.tex <==
//Old Comment: Returns an java.time.Instant object that is offset by a number of milliseconds from now.
public static Instant getInstantMillisOffsetFromNow(long offsetInMillis) {
    return Instant.now().plus(Duration.ofMillis());
}

//New Comment for the changed code: Returns an java.time.Instant object that is offset by a number of hours from now
public static Instant getInstantHoursOffsetFromNow(long offsetInHours) {
    return Instant.now().plus(Duration.ofHours());
}

==> code/commit_message.tex <==
cd ../
git clone https://github.com/facebook/wangle.git
cd wangle/wanglegit checkout ...
-cmake .
+cmake . -DBUILD_TESTS=OFF
ctest
sudo make install


==> code/log_anomaly.tex <==
Jun 14 15:16:01 combo sshd(pam_unix)[19939]: authentication failure; logname= uid=0 euid=0 tty=NODEVssh ruser= rhost=218.188.2.4 
Jun 14 15:16:02 combo sshd(pam_unix)[19937]: check pass; user unknown
Jun 14 15:16:02 combo sshd(pam_unix)[19937]: authentication failure; logname= uid=0 euid=0 tty=NODEVssh ruser= rhost=218.188.2.4 
...

==> code/quality_exception.tex <==
// target code
public boolean equals(Object other) {
    try {
        if (other == null) {
            return false;
        }
        return d.equals(((BigReal) other).d);
    } catch (ClassCastException cce) {
        return false;
    }
}

// runtime exception detection by ChatGPT
// 1. NullPointerException: ...
// 2. ClassCastException: ... (ground-truth)
// 3. Missing null check: ...
// 4. Precision loss: ...
// To improve this code, it may be ...

==> code/testcase_generation.tex <==
// focal test:
testReportErrorOnWrongDateEffective () {
    java.lang.String drl ="rule_X_date-effective_\"9-asbrdfh-1974\"_when\n" + (("\$s:_String()"+"then\n") + "end\n") ;
    org.kie.internal.builder.KnowledgeBuilder kb = org.kie.internal.builder.KnowledgeBuilderFactory.newKnowledgeBuilder();
    kb.add(new org.drools.core.io.impl.ByteArrayResource(drl.getBytes()), ResourceType.DRL);
}
hasErrors(){
    return (errors)!=null;
}

// The assertion generated by ChatGPT is same as the ground-truth:
org.junit.Assert.assertTrue(kb.hasErrors())

==> exp.tex <==
\subsection{Baselines}\label{sec_baseline}



\subsection{Research Questions}\label{sec_rq}

In this study, we proposed a method to guide ChatGPT for two code generation tasks. To verify the effectiveness of the method and analyze the associated influential factors, this study investigated the following RQs:

\RQ{1}{How effective is the designed prompt for ChatGPT?}

We designed a prompt framework to guide ChatGPT for better code generation. To verify the effectiveness of the prompt framework, we tested on the two datasets described in Section \ref{sec_dataset} and compared the performance with other baselines as referred to in Section \ref{sec_baseline}.

\RQ{2}{How the prompt components affect ChatGPT?}

As illustrated in Section \ref{sec_framework}, our designed prompt framework consists of \bl{xxx} components, including role, context, task, response, and format. This RQ aims to investigate how these components affect the generation performance. To reach the goal, we removed each component respectively and assessed generation performance.

\RQ{3}{How the prompt complexity affects ChatGPT?}

Our designed prompt is complex with all detailed descriptions. It is reasonable to consider whether a detailed description is necessary for ChatGPT. To answer this RQ, we asked ChatGPT to help us provide \bl{xxx} types of concise prompts. We guided ChatGPT with these prompts respectively and assessed the code generation performance.

\RQ{4}{How the session size affects ChatGPT?}

As ChatGPT has the ability to remember chatting context within a session, the objective of this RQ is to investigate how different session sizes affect the code generation performance. To conduct the experiment, we tested the guided ChatGPT with a fixed number of testing data, where the number was adopted from the set \bl{\{1, 2, 5, 10, 20\}}. As the session size is limited by ChatGPT API, we did not test the larger numbers.

\RQ{5}{How the generation randomness affects ChatGPT?}

It is known that ChatGPT may generate code with slight difference every time for the same prompt. To investigate how the randomness affect the generation performance, we reran the guided-ChatGPT \bl{ten} times in total and analyzed the stability of the generation performance.
